Nonlinear Heterogeneous Bayesian Decentralized Data Fusion

The factor graph decentralized data fusion (FG-DDF) framework was developed for the analysis and exploitation of conditional independence in {heterogeneous Bayesian decentralized fusion problems, in which robots update and fuse pdfs over different, but overlapping subsets of random states. This allows robots to efficiently use smaller probabilistic models and sparse message passing to accurately and scalably fuse relevant local parts of a larger global joint state pdf while accounting for data dependencies between robots. Whereas prior work required limiting assumptions about network connectivity and model linearity, this paper relaxes these to explore the applicability and robustness of FG-DDF in more general settings. We develop a new heterogeneous fusion rule which generalizes the homogeneous covariance intersection algorithm for such cases and test it in multi-robot tracking and localization scenarios with non-linear motion/observation models under communication dropouts. Simulation and hardware experiments show that, in practice, the FG-DDF continues to provide consistent filtered estimates under these more practical operating conditions, while reducing computation and communication costs by more than 99\%, thus enabling the design of scalable real-world multi-robot systems.

==> Text/Some_Ideas.tex <==
\begin{itemize}
    \item \textbf{Goal:} The Goal of this work is to show the scalability and test the limits of the FG-DDF framework.
    
    %The goal of this work is to empirically explore the nonlinear heterogeneous DDF filtering problem and surface gaps.
    \item \textbf{Application}: Decentralized target tracking and localization (not CL) of a heterogeneous multi-agent team.
    \item \textbf{Possible avenues to explore (in the future):} Static with nonlinear measurements; \od{linear dynamics/nonlinear measurement}; nonlinear dynamics/linear measurements; \od{full nonlinear}. 
    
    \item Comparison of decentralized results to the true pdf and to centralized requires:
    \begin{itemize}
        \item Centralized particle filter
        \item Centralized EKF
    \end{itemize}
    \item Comparing CF to CI 
    \item KLD to the true pdf?
    \item Timing / complexity?
    \item Non full rate
\end{itemize}

\textbf{Relevant Papers:}
\begin{itemize}
    \item \cite{ahmad_cooperative_2013} - NLS solution for coop-localization and target tracking + experimental results
    \item \cite{ong_decentralised_2008} - CF using PF for target tracking
    \item \cite{fernandes_cooperative_2020} - Coop localization using factor graphs
    \item \cite{zhu_fully_2020} - distributed joint localization and tracking
    \item \cite{lyu_collaborative_2018} - Collaborative localization and tracking (CLAT).
\end{itemize}




